Neural Collapse Meets Differential Privacy: Curious Behaviors of NoisyGD with Near-perfect Representation Learning

A recent study by De et al. (2022) has reported that large-scale representation learning through pre-training on a public dataset significantly enhances differentially private (DP) learning in downstream tasks, despite the high dimensionality of the feature space. To theoretically explain this phenomenon, we consider the setting of a layer-peeled model in representation learning, which results in interesting phenomena related to learned features in deep learning and transfer learning, known as Neural Collapse (NC). Within the framework of NC, we establish an error bound indicating that the misclassification error is independent of dimension when the distance between actual features and the ideal ones is smaller than a threshold. Additionally, the quality of the features in the last layer is empirically evaluated under different pre-trained models within the framework of NC, showing that a more powerful transformer leads to a better feature representation. Furthermore, we reveal that DP fine-tuning is less robust compared to fine-tuning without DP, particularly in the presence of perturbations. These observations are supported by both theoretical analyses and experimental evaluation. Moreover, to enhance the robustness of DP fine-tuning, we suggest several strategies, such as feature normalization or employing dimension reduction methods like Principal Component Analysis (PCA). Empirically, we demonstrate a significant improvement in testing accuracy by conducting PCA on the last-layer features.

==> figures/preliminary.tex <==

\section{Preliminaries}
\label{sec:preliminary}

In this section, we review the private fine-tuning literature, introduce the Neural Collapse phenomenon and formalize the private fine-tuning set up. We start by defining differential privacy \citep{dwork2006differential}.


% \subsection{Differential privacy}
Differential privacy (DP) requires the output of an algorithm to be indistinguishable upon the change of an individual training data point.
Mathematically, let $\mathcal{D} = \{z_i\}_{i=1}^n\subset \mathcal{Z}$ be a fixed dataset of size $n$ and consider a randomized algorithm $\mathcal{A}:\mathcal{Z}^n \rightarrow \mathcal{S}$ that maps a dataset $\mathcal{D}$ to $\mathcal{A}(\mathcal{D}) $ in some probability space $\mathcal{S}$.
We say $\mathcal{A}$ satisfies $(\epsilon,\delta)$-DP for some $\epsilon\geq 0$ and $0\leq \delta \leq 1$ if 
$
    \mathbb{P}[\mathcal{A}(\mathcal{D}_0)\in S]\leq e^{\epsilon}\mathbb{P}[\mathcal{A}(\mathcal{D}_1)\in S]  + \delta,
$
for any event $S\in\mathcal{S}$ and any neighboring datasets $\mathcal{D}_0$ and $\mathcal{D}_1$. 

\begin{definition}[Zero-Concentrated Differential Privacy, zCDP, \citet{DBLP:conf/tcc/BunS16}]
A randomized mechanism $\cA$ satisfies $\rho$-zero-concentrated differentially private ($\rho$-zCDP) if, for all neighboring datasets $\cD_0$ and $\cD_1$, we have
$
    R_{\alpha}(\mathcal{A}(\cD_0)\|\cA(\cD_1)) \leq \rho \alpha,
$
where $  R_{\alpha}(P\|Q) = \frac{1}{\alpha - 1} \log \int \left(\frac{p(x)}{q(x)} \right)^{\alpha} q(x) dx$ is the R\'enyi divergence between two distributions $P$ and $Q$.
\end{definition}

Our privacy analysis is based on the $\rho$-zCDP framework, which often allows for a tighter $(\epsilon,\delta)$-DP over compositions and we can convert $\rho$-zCDP to $(\epsilon, \delta)$-DP for any $\delta$.
% Our analysis is based on $\rho$-zCDP which is defined based on the R\'enyi divergence between $\mathcal{A}(\mathcal{D}_0)$ and $\mathcal{A}(\mathcal{D}_1).$
% The R\'enyi divergence of order $\widetilde{\alpha}>1$ between $P$ and $Q$ is given by
% \begin{align*}
%   R_{\widetilde{\alpha}}(P\|Q) = \frac{1}{\widetilde{\alpha} - 1} \log \int \left(\frac{p(x)}{q(x)} \right)^{\widetilde{\alpha}} q(x) dx.
% \end{align*}
% For ${\widetilde{\alpha}} =1$ or $+\infty$, $R_1$ or $R_{\infty}$ is the limit of $R_{\widetilde{\alpha}}$ as $\widetilde{\alpha}$ tends to $1$ or $+\infty$.
% With a little bit abuse of notations, we define the R\'enyi divergence between two random variables as the divergence between their distributions.
% Then, an algorithm is said to satisfy $\rho$-zCDP if 
% $
% R_{\widetilde{\alpha}}\left(\mathcal{A}(\mathcal{D}_0) \| \mathcal{A}(\mathcal{D}_1)\right) \leq \rho \widetilde{\alpha}
% $
% for any neighboring datasets $\mathcal{D}_0$ and $\mathcal{D}_1$ and any $1<\widetilde{\alpha}<\infty$.



\textbf{Noisy gradient descent.}
Noisy Gradient Descent (NoisyGD) or its stochastic version Noisy Stochastic Gradient Descent (NoisySGD, \citet{song2013stochastic,abadi2016DPSGD}) is a fundamental algorithm in DP deep learning. 
To minimize the loss function $\cL(\theta) := \sum_{i=1}^n \ell(\theta, z_i)$, the NoisyGD algorithm updates the model parameter $\theta_t$ by combining the gradient with an isotropic Gaussian.
\begin{align}
\label{eq:DP-GD}
 \theta_{t+1} = \theta_t - \eta_t \left(\sum_{i=1}^n \nabla \ell(\theta_t, z_i) + \cN\left(0, \frac{G^2}{2\rho} I_p\right) \right).
 \end{align}
Here $G$ is the $\ell_2$-sensitivity of the gradient, and the algorithm runs for $T$ iterations satisfies $T\rho$-zCDP.


However, the excess risk of NoisySGD must grow as $\sqrt{p}/\epsilon$ \citep{DBLP:conf/focs/BassilyST14}, which limits private deep learning benefit from model scales. To overcome this, DP fine-tuning \citep{de2022unlocking, li2021large, bu2022differentially} is emerging as a promising approach to train large models with privacy guarantee.

%\noindent\textbf{Why do we consider fine-tuning the last layer?}
\noindent\textbf{Private fine-tuning.}
In DP fine-tuning, we begin by pre-training a model on a public dataset and then privately fine-tuning the pre-trained model on the private dataset. Our focus is on fine-tuning the last-layer of pre-trained models using the NoisySGD/NoisyGD algorithm, which has consistently achieved state-of-the-art results across both vision and language classification tasks~\citep{de2022unlocking, tramer2020differentially, bao2023dpmix}. However, we acknowledge that in some scenarios, fine-tuning all layers under DP can result in better performance, as demonstrated in the CIFAR-10 task by \citet{de2022unlocking}. The comprehensive analysis of dimension-dependence in other private fine-tuning benchmarks remains an area for future investigation.
%From a Neural Collapse perspective, it is intriguing to explore the impact of DP fine-tuning on the last-layer feature when fine-tuning all layers, a subject that will be further investigated in our future research.

%as this approach yields higher accuracy compared to fine-tuning all layers. This is supported by  Figure 4 and 5 in \citet{de2022unlocking}, which involve pre-training on JFT-300M or JFT-4B and fine-tuning on ImageNet
%A recent study by \citet{bao2023dpmix} has similarly observed that fine-tuning only the final layer can result in high accuracy.
%Hence, our theoretical framework in this paper centered on exclusively fine-tuning the last layer, which covers a wide range of practical scenarios.




\noindent\textbf{Theoretical setup for private fine-tuning.}
For a $K$-class classification task, we rewrite each data point $z$ as $z= (x,y)$ with $x\in\mathbb{R}^p$ being the feature and $y = (y_1,\cdots, y_K)\in\{0,1\}^K$ being the corresponding label generated by the one-hot encoding, that is $y$ belongs to the $k$-th class if $y_k = 1$ and $y_j = 0$ for $j\neq k.$

When applying NoisyGD for fine-tuning the last-layer parameters, the model is in a linear form. 
Thus, we consider the linear model $f_{W}(x) = W x$ with $W\in\mathbb{R}^{K\times p}$ being the last-layer parameter to be  trained and $x$ is the last layer feature of a data point.
The parameter $\theta_t$ in NoisyGD is the vectorization of $W$.
Let $\ell:\mathbb{R}^K \times \mathbb{R}^K\rightarrow \mathbb{R}$ be a loss function that maps $f_{W}(x) \in \mathbb{R}^K$ and the label $y$ to $\ell(f_W(x), y).$
For example, for the cross-entropy loss, we have $\ell(f_W(x), y) = -\sum_{i=1}^K y_i\log[(f_W(x))_i].$



\paragraph{Mis-classification error.}
For an output $\widehat{W}$ and a testing data point $(x,y)$, the mis-classification error is defined as $\mathbb{P}\left[y\neq \mathrm{OneHot}\left(f_{\widehat{W}}(x)\right)\right],$ where the probability is taken with respect to the randomness of $\widehat{W}$ and $(x,y).$

Bounding the mis-classification error directly is challenging in general due to the non-convex nature of the 0-1 loss.
Thus, most existing research relies on the comparison theorem \cite{MR2268032,MR2248013} to establish bounds on the misclassification error, which essentially investigates the excess risk of the convex surrogate loss. Nevertheless, by utilizing Neural Collapse techniques, we can study the misclassification error directly, without using a convex surrogate loss.


%To investigate the mis-classification error based on the last layer features, we relate the feature quality to Neural Collapse.
%By adopting Neural Collapse, we define the perfect feature for the $k$-th class as the $k$ the column of an equiangular tight frame (ETF).
%It has been widely observed that the mean of the last layer feature converges to an ETF \citep{DBLP:journals/corr/abs-2008-08186, fang2021exploring,doi:10.1073/pnas.2221704120}.

\noindent\textbf{Neural Collapse.}
Neural Collapse~\citep{DBLP:journals/corr/abs-2008-08186, fang2021exploring,doi:10.1073/pnas.2221704120} describes a phenomenon about the last-layer feature structure obtained when a deep classifier neural network converges. It  demonstrates that the last-layer feature converges to the column of an equiangular tight frame (ETF). 
Mathematically, an ETF is a matrix 
\begin{align}
\label{eq:defn-etf}
    M &= \sqrt{\frac{K}{K-1}} P \left(I_K - \frac{1}{K}\mathbf{1}_K \mathbf{1}_K^T\right) \in\mathbb{R}^{p\times K},
\end{align}
where $P=[P_1,\cdots, P_K]\in\mathbb{R}^{p\times K}$ is a partial orthogonal matrix such that $P^T P = I_K$. For a given dimension $d=p$ or $K$, we denote $I_d\in\mathbb{R}^d$ the identity matrix and denote $\mathbf{1}_d=[1,\cdots, 1]^T\in\mathbb{R}^d$.
Rewrite $M = [M_1,\cdots, M_K]$ with $M_k$ being the $k$-th column of $M$, that is,  the feature of the data belonging to class $k$.
%We define the classification problem under perfect Neural Collapse as follows.

%For the $k$-th class, we call $M_k$ the perfect feature.

We utilize the Neural Collapse theory to describe an ideal feature representation of applying the pre-trained model on the private set.  However, achieving perfect collapse on the private set is an ambitious assumption, as in practice, the private feature of a given class is distributed around $M_k$. Therefore, we introduce a feature shift parameter $\beta$ to measure the discrepancy between the actual feature and the perfect feature $M_k$.



%Thus, it is reasonable to regard it as the perfect feature.
%However, achieving perfect collapse is rarely feasible in practical applications. Typically, the features of a given class are distributed around $M_k$. Therefore, we quantify the feature quality by the distance between true features and the perfect one.

\begin{definition}[Feature shift parameter $\beta$] For any $1\leq k \leq K$, given a feature $x$ belonging to the $k$-th class and the perfect feature $M_k$,  we define $\beta =  ||x- M_k ||_{\infty}$ as the feature shift parameter of $x$ that measures the $\ell_{\infty}$ distance between $x$ and $M_k$.
\end{definition}

%{\color{red}
%We study the $\ell_{\infty}$ distance since it is related to the adversarial robustness of DP fine-tuning.
%This is due to the fact that an adversarial attacker will increase this $\ell_{\infty}$ distance, thus challenging the model's robustness.
%}

% \subsection{Private fine-tuning}
% Th
% One popular application of NoisyGD is private fine-tuning, which 


% % Note that when $K=2$, we have $M_1 = -M_2$, where the features corresponding to different classes are linearly dependent.

% % \begin{definition}[Classification problem under prefect Neural Collapse]
% % \label{defn:NC}
% % 	Let there be $K$ classes. The distribution $\P[x  = M_k|y_k = 1]  = 1$ for $k=1,...,K$. 
% % \end{definition} 




% Denote $\mathcal{N}(0,\sigma^2 I_d)$ a Gaussian random variable in $\mathbb{R}^d$ with covariance matrix $\sigma^2 I_d.$
% Let $\theta \in \mathbb{R}^p$ be the vectorization of the parameters.
% With a little bit abuse of notations, we rewrite $\ell_i(\theta) = \ell(\theta, z_i)$ the loss function with respect to the data point $z_i.$
% The noisy gradient descent is defined as follows.

% \textbf{Noisy Stochasitic Gradient Descent (NoisySGD).}
% Let the loss function $\cL(\theta) := \sum_{i=1}^n \ell(\theta, z_i)$. The noisy gradient descent algorithm outputs
% \begin{align*}
%  \theta_{t+1} = \theta_t - \frac{\eta_t}{|\mathcal{B}_t|} \left(\sum_{z_i\in\mathcal{B}_t} \nabla \ell_i(\theta_t) + \cN\left(0, \frac{G^2}{2\rho} I_d\right) \right).
%  \end{align*}
% % \begin{align*}
% %  \theta_{t+1} = \theta_t - \frac{\eta_t}{|\mathcal{B}_t|} \left(\sum_{z_i\in\mathcal{B}_t} \max\left\{1, \frac{G}{\|\nabla \ell_i(\theta_t)\|_2}\right\}\nabla \ell_i(\theta_t) + \cN\left(0, \frac{G^2}{2\rho} I_d\right) \right).
% %  \end{align*}
%  Here $\mathcal{B}_t$ is a mini-batch selected uniformly at random in the $t$-th step and $G$ is the $\ell_2$-sensitivity of the gradient.
% The algorithm that runs the above for $T$ iterations satisfies $T\rho$-zCDP \citep{abadi2016DPSGD}.

% When $\mathcal{B}_t$ represents the entire training set, the NoisySGD algorithm reduces to a Noisy Gradient Descent (NoisyGD) algorithm. 
% In our experiments, we use NoisySGD to enhance the efficiency.
% Our theory focuses on the NoisyGD.



% \textbf{Noisy Gradient Descent (NoisyGD).}
% Let the loss function $\cL(\theta) := \sum_{i=1}^n \ell(\theta, z_i)$. The noisy gradient descent algorithm outputs
% \begin{align}
% \label{eq:DP-GD}
%  \theta_{t+1} = \theta_t - \eta_t \left(\sum_{i=1}^n \nabla \ell_i(\theta_t) + \cN\left(0, \frac{G^2}{2\rho} I_d\right) \right).
%  \end{align}
%  Here $G$ is the $\ell_2$-sensitivity of the gradient.



==> macro_yuxiang.tex <==
\usepackage{amsmath,amsthm,amssymb,bbm}
\usepackage{mathtools}
\usepackage{cases}
\usepackage{dsfont}
\usepackage{microtype}

\newcommand{\explain}[2]{\underset{\mathclap{\overset{\uparrow}{#2}}}{#1}}
\newcommand{\explainup}[2]{\overset{\mathclap{\underset{\downarrow}{#2}}}{#1}}


\usepackage{amsmath}
\newcommand\norm[1]{\left\lVert#1\right\rVert}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand{\minimize}{\mathop{\mathrm{minimize}}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\defeq}{\mathrel{\mathop:}=}


%\newcommand{\E}{\mathop{\mathbb{E}}}
\def\tin{\text{in}}
\def\PP{\textit{\textbf{P}}}
\def\hpi{\widehat{\pi}}
\def\E{\mathbb{E}}
\def\P{\mathbb{P}}
\def\Cov{\mathrm{Cov}}
\def\Var{\mathrm{Var}}
\def\half{\frac{1}{2}}
\def\th{\mathrm{th}}
\def\tr{\mathrm{tr}}
\def\df{\mathrm{df}}
\def\dim{\mathrm{dim}}
\def\col{\mathrm{col}}
\def\row{\mathrm{row}}
\def\nul{\mathrm{null}}
\def\rank{\mathrm{rank}}
\def\nuli{\mathrm{nullity}}
\def\sign{\mathrm{sign}}
\def\supp{\mathrm{supp}}
\def\diag{\mathrm{diag}}
\def\aff{\mathrm{aff}}
\def\hy{\hat{y}}
\def\ty{\tilde{y}}
\def\hbeta{\hat{\beta}}
\def\tbeta{\tilde{\beta}}
\def\htheta{\hat{\theta}}
\def\halpha{\hat{\alpha}}
\def\hf{\hat{f}}
\def\lone{1}
\def\ltwo{2}
\def\linf{\infty}
\def\lzero{0}
\def\T{^T}
\def\R{\mathbb{R}}
\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cP{\mathcal{P}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}
\def\TV{\mathrm{TV}}

